DNN-GDITD: Out-of-distribution detection via Deep Neural Network based Gaussian Descriptor for Imbalanced Tabular Data

Classification tasks present challenges due to class imbalances and evolving data distributions. Addressing these issues requires a robust method to handle imbalances while effectively detecting out-of-distribution (OOD) samples not encountered during training. This study introduces a novel OOD detection algorithm designed for tabular datasets, titled Deep Neural Network-based Gaussian Descriptor for Imbalanced Tabular Data (DNN-GDITD). The DNN-GDITD algorithm can be placed on top of any DNN to facilitate better classification of imbalanced data and OOD detection using spherical decision boundaries. Using a combination of Push, Score-based, and focal losses, DNN-GDITD assigns confidence scores to test data points, categorizing them as known classes or as an OOD sample. Extensive experimentation on tabular datasets demonstrates the effectiveness of DNN-GDITD compared to three OOD algorithms. Evaluation encompasses imbalanced and balanced scenarios on diverse tabular datasets, including a synthetic financial dispute dataset and publicly available tabular datasets like Gas Sensor, Drive Diagnosis, and MNIST, showcasing DNN-GDITD's versatility.

==> table_class_copy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
\begin{table*}%[hbt!]
\caption{Comparison of proposed DNN-GDID with Softmax \cite{softmax}, Mahalanobis \cite{lee2018simple} and Deep-MCDD \cite{deep_mcdd} (Best in bold).}
\label{table_class}
\resizebox{12.85cm}{!}
{
\begin{tabular}{|c|cccccc|}
\hline
\multirow{3}{*}{Dataset}                          & \multicolumn{1}{c|}{MDR}  & \multicolumn{1}{c|}{\textbf{ID class}}       & \multicolumn{3}{c|}{\textbf{OOD class}}                                                                                                                                         &\textbf{Minority class} \\ \cline{2-7} 
& \multicolumn{6}{c|}{Softmax ~\cite{softmax} \textbf{\textbar} Mahalanobis ~\cite{lee2018simple} \textbf{\textbar} Deep-MCDD ~\cite{deep_mcdd} \textbf{\textbar} DNN-GDID (ours)}                                                                                                                                                                                                            \\ \cline{2-7} 
& \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{Classification accuracy} & \multicolumn{1}{c|}{TNR at 85\% TPR}      & \multicolumn{1}{c|}{AUROC}                 & \multicolumn{1}{c|}{AUPR}                   & AUPR                    \\ \hline\hline
% #-------------SYN FINANCIAL ------------------
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Synthetic \\ financial\\ Dataset\end{tabular}}               & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{\textbf{99.45}\textbf{\textbar}97.68\textbf{\textbar} 99.31\textbf{\textbar}99.34}    & \multicolumn{1}{c|}{43.93\textbf{\textbar}50.96\textbf{\textbar} 83.90\textbf{\textbar}\textbf{86.01}} & \multicolumn{1}{c|}{48.43\textbf{\textbar}78.09\textbf{\textbar} 90.65\textbf{\textbar}\textbf{91.45}}  & \multicolumn{1}{c|}{86.12\textbf{\textbar}93.57\textbf{\textbar}97.39\textbf{\textbar}\textbf{97.53}}    & 98.59\textbf{\textbar}15.80\textbf{\textbar} 99.31\textbf{\textbar}\textbf{99.33}    \\ \cline{2-7} 
%-------SYN FINANCIAL---- 0.30 ----------------------------------
& \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\textbf{99.41}\textbf{\textbar}98.04\textbf{\textbar} 99.21\textbf{\textbar}99.34}                & \multicolumn{1}{c|}{47.20\textbf{\textbar}61.69\textbf{\textbar}84.36\textbf{\textbar}\textbf{89.09}}              & \multicolumn{1}{c|}{45.47\textbf{\textbar}80.16\textbf{\textbar}  90.73\textbf{\textbar}\textbf{93.22}}             & \multicolumn{1}{c|}{86.97\textbf{\textbar}95.09\textbf{\textbar}  97.69\textbf{\textbar}\textbf{98.34}}                   & 95.87\textbf{\textbar}04.44\textbf{\textbar}96.33\textbf{\textbar}\textbf{96.56}               \\ \cline{2-7}
%---------SYN FINANCIAL--- 0.25 ----------------------------------
& \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{\textbf{99.43}\textbf{\textbar}92.08\textbf{\textbar}99.22\textbf{\textbar}99.34}           & \multicolumn{1}{c|}{44.99\textbf{\textbar}52.44\textbf{\textbar}84.79\textbf{\textbar}\textbf{87.16}}       & \multicolumn{1}{c|}{45.40\textbf{\textbar}75.10\textbf{\textbar} 90.29\textbf{\textbar}\textbf{92.13}}              & \multicolumn{1}{c|}{86.83\textbf{\textbar}93.55\textbf{\textbar} 97.70\textbf{\textbar}\textbf{98.00}}                        & 94.47\textbf{\textbar}04.95\textbf{\textbar} 94.97\textbf{\textbar}\textbf{95.66}               \\ \hline
% \\ \cline{2-7} 
% %-------SYN FINANCIAL--- 0.20 ----------------------------------
% & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{99.44\textbf{\textbar}\textbf{\textbar} 99.28\textbf{\textbar}99.34}                & \multicolumn{1}{c|}{48.04\textbf{\textbar}\textbf{\textbar} 88.16\textbf{\textbar}84.58}             & \multicolumn{1}{c|}{47.55\textbf{\textbar}\textbf{\textbar} 92.66\textbf{\textbar}89.90}              & \multicolumn{1}{c|}{87.84\textbf{\textbar}\textbf{\textbar} 98.17\textbf{\textbar}97.58}                          &94.70\textbf{\textbar}\textbf{\textbar} 93.85\textbf{\textbar}93.49               \\ \cline{2-7}
% %--------SYN FINANCIAL--- 0.15 ----------------------------------
% & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{99.52\textbf{\textbar}\textbf{\textbar} 99.37\textbf{\textbar}99.44}                & \multicolumn{1}{c|}{47.02\textbf{\textbar}\textbf{\textbar}86.38 \textbf{\textbar}84.71}             & \multicolumn{1}{c|}{45.94\textbf{\textbar}\textbf{\textbar} 91.36\textbf{\textbar}90.58}              & \multicolumn{1}{c|}{87.52\textbf{\textbar}\textbf{\textbar} 98.05\textbf{\textbar}97.73}                        &92.14\textbf{\textbar}\textbf{\textbar} 92.11\textbf{\textbar}90.86               \\ \cline{2-7} 
% %-------SYN FINANCIAL-- 0.10 ----------------------------------
% & \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{99.58\textbf{\textbar}98.40\textbf{\textbar}99.46\textbf{\textbar}99.49 }                & \multicolumn{1}{c|}{49.76\textbf{\textbar}51.31\textbf{\textbar}87.74\textbf{\textbar}85.10}             & \multicolumn{1}{c|}{48.67\textbf{\textbar}81.42\textbf{\textbar}92.67\textbf{\textbar}91.44}              & \multicolumn{1}{c|}{88.43\textbf{\textbar}94.98\textbf{\textbar}98.31\textbf{\textbar}97.89}                          & 90.10\textbf{\textbar} 4.68\textbf{\textbar}89.37\textbf{\textbar} 87.59              \\ \hline
% #------------ GAS SENSOR --------------------
\multicolumn{1}{|c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Gas \\ Sensor \\ Dataset \\ ~\cite{data_gas}\end{tabular}} } & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{\textbf{99.67}\textbf{\textbar}90.65\textbf{\textbar} 99.61\textbf{\textbar} 99.66}     & \multicolumn{1}{c|}{45.59\textbf{\textbar}88.08\textbf{\textbar} 93.13\textbf{\textbar}\textbf{97.62}} & \multicolumn{1}{c|}{60.24\textbf{\textbar}92.75\textbf{\textbar} 95.88\textbf{\textbar}\textbf{97.59}}  & \multicolumn{1}{c|}{72.44\textbf{\textbar}90.70\textbf{\textbar}  95.43\textbf{\textbar}\textbf{97.19}}  & 99.61\textbf{\textbar}24.81\textbf{\textbar}\textbf{99.63}\textbf{\textbar}99.60   \\ \cline{2-7} 
%----------------------- GAS SENSOR-- 0.30 ------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\textbf{99.70}\textbf{\textbar}97.65\textbf{\textbar} 99.69\textbf{\textbar}99.68}    & \multicolumn{1}{c|}{40.34\textbf{\textbar}87.80\textbf{\textbar} 93.51\textbf{\textbar}\textbf{93.64}} & \multicolumn{1}{c|}{57.16\textbf{\textbar}92.53\textbf{\textbar}  95.98\textbf{\textbar}\textbf{96.04}} & \multicolumn{1}{c|}{71.78\textbf{\textbar}91.79\textbf{\textbar}\textbf{96.29}\textbf{\textbar}95.98}   &\textbf{98.05}\textbf{\textbar}06.32\textbf{\textbar} 97.69\textbf{\textbar}\textbf{98.05 }   \\ \cline{2-7} 
%--------------- GAS SENSOR-- 0.25 -------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{99.68\textbf{\textbar}97.48\textbf{\textbar}\textbf{99.70}\textbf{\textbar}99.68}    & \multicolumn{1}{c|}{40.02\textbf{\textbar}90.03\textbf{\textbar} 93.69\textbf{\textbar}\textbf{94.15}} & \multicolumn{1}{c|}{56.13\textbf{\textbar}93.15\textbf{\textbar} 95.88\textbf{\textbar}\textbf{96.07}}  & \multicolumn{1}{c|}{70.86\textbf{\textbar}93.60\textbf{\textbar} 95.85\textbf{\textbar}\textbf{96.21}}   & 97.08\textbf{\textbar}05.27\textbf{\textbar}\textbf{98.05}\textbf{\textbar}97.95    \\ \cline{2-7}
%------------ GAS SENSOR--- 0.20 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{\textbf{99.68}\textbf{\textbar}97.76\textbf{\textbar} 99.67\textbf{\textbar}99.64}    & \multicolumn{1}{c|}{45.16\textbf{\textbar}92.23\textbf{\textbar}93.94\textbf{\textbar}\textbf{94.70}}  & \multicolumn{1}{c|}{60.36\textbf{\textbar}93.66\textbf{\textbar} 96.00\textbf{\textbar}\textbf{96.62}}  & \multicolumn{1}{c|}{74.61\textbf{\textbar}92.97\textbf{\textbar}96.09\textbf{\textbar}\textbf{96.51}}    & 97.44\textbf{\textbar}04.36\textbf{\textbar}\textbf{97.59}\textbf{\textbar}97.35    \\ \cline{2-7} 
%---------- GAS SENSOR--- 0.15 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{99.67\textbf{\textbar}79.18\textbf{\textbar}\textbf{99.71}\textbf{\textbar}99.70}    & \multicolumn{1}{c|}{36.44\textbf{\textbar}79.06\textbf{\textbar}84.34\textbf{\textbar}\textbf{96.61}} & \multicolumn{1}{c|}{57.20\textbf{\textbar}87.33\textbf{\textbar} 92.35\textbf{\textbar}\textbf{97.11}}  & \multicolumn{1}{c|}{70.18\textbf{\textbar}89.21\textbf{\textbar} 92.64\textbf{\textbar}\textbf{97.04}}  &96.71\textbf{\textbar}03.04\textbf{\textbar} 96.23\textbf{\textbar}\textbf{96.76}    \\ \cline{2-7} 
%---------- GAS SENSOR--- 0.10 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{99.68\textbf{\textbar}78.81\textbf{\textbar} 99.71\textbf{\textbar}\textbf{99.72}}          & \multicolumn{1}{c|}{41.76\textbf{\textbar}91.70\textbf{\textbar} 84.34\textbf{\textbar}\textbf{93.99}}       & \multicolumn{1}{c|}{58.60\textbf{\textbar}93.18\textbf{\textbar} 92.35\textbf{\textbar}\textbf{96.12}}        & \multicolumn{1}{c|}{72.06\textbf{\textbar}93.63\textbf{\textbar} 92.64\textbf{\textbar}\textbf{96.28}}             & 96.00\textbf{\textbar}01.91\textbf{\textbar}\textbf{96.23}\textbf{\textbar}\textbf{96.23}          \\ \hline

%--------------------  Drive Diagnosis ------------------------------------
\multirow{5}{*}{{\begin{tabular}[c]{@{}c@{}} Drive \\ Diagnosis \\ Dataset \\ ~\cite{data_drive}\end{tabular}}}                  & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{99.70\textbf{\textbar} 99.76\textbf{\textbar}95.22\textbf{\textbar}\textbf{99.81}}   & \multicolumn{1}{c|}{15.45\textbf{\textbar}41.95\textbf{\textbar} 63.56\textbf{\textbar}\textbf{66.54}}       & \multicolumn{1}{c|}{23.52\textbf{\textbar}78.87\textbf{\textbar}80.29\textbf{\textbar}\textbf{83.43}}        & \multicolumn{1}{c|}{28.82\textbf{\textbar}54.48\textbf{\textbar} 70.31\textbf{\textbar}\textbf{71.44}}            & 99.71\textbf{\textbar}21.90\textbf{\textbar}99.83\textbf{\textbar}\textbf{ 99.85}        \\ \cline{2-7}
%------Drive Diagnosis--- 0.30 ----------------------------------
& \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{99.73\textbf{\textbar}94.73\textbf{\textbar} 99.79\textbf{\textbar}\textbf{99.82}}    & \multicolumn{1}{c|}{15.68\textbf{\textbar}38.30\textbf{\textbar}60.33\textbf{\textbar}\textbf{70.08}}  & \multicolumn{1}{c|}{22.50\textbf{\textbar}  79.37\textbf{\textbar}77.02\textbf{\textbar}\textbf{84.94}} & \multicolumn{1}{c|}{29.71\textbf{\textbar}54.33\textbf{\textbar}  69.98\textbf{\textbar}\textbf{74.47}} &  99.48\textbf{\textbar}04.83\textbf{\textbar} 99.43\textbf{\textbar}\textbf{99.53}     \\ \cline{2-7} 
%---Drive Diagnosis---- 0.25 ----------------------------------
& \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{99.70\textbf{\textbar}94.77\textbf{\textbar} 99.78\textbf{\textbar}\textbf{99.79}}          & \multicolumn{1}{c|}{16.19\textbf{\textbar}32.99\textbf{\textbar} 53.79\textbf{\textbar}\textbf{64.90}}       & \multicolumn{1}{c|}{22.39\textbf{\textbar}75.22\textbf{\textbar} 75.31\textbf{\textbar}\textbf{82.85}}        & \multicolumn{1}{c|}{30.02\textbf{\textbar}52.18\textbf{\textbar} 66.13\textbf{\textbar}\textbf{71.94}}     & 98.96\textbf{\textbar}04.67\textbf{\textbar} 99.47\textbf{\textbar}\textbf{99.48 }        \\ \cline{2-7} 
%-------Drive Diagnosis---- 0.20 ----------------------------------
& \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{99.73\textbf{\textbar}95.09\textbf{\textbar} 99.79\textbf{\textbar}\textbf{99.81}}          & \multicolumn{1}{c|}{17.79\textbf{\textbar}43.76\textbf{\textbar} 66.61\textbf{\textbar}\textbf{70.20}}       & \multicolumn{1}{c|}{26.48\textbf{\textbar}77.95\textbf{\textbar}82.97\textbf{\textbar}\textbf{85.44}}        & \multicolumn{1}{c|}{32.51\textbf{\textbar}57.47\textbf{\textbar} 74.30\textbf{\textbar}\textbf{75.76}}        &  98.75\textbf{\textbar}04.53\textbf{\textbar}\textbf{99.33}\textbf{\textbar}99.32          \\ \cline{2-7} 
%------Drive Diagnosis----- 0.15 ----------------------------------
& \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{99.70\textbf{\textbar}94.89\textbf{\textbar} 99.74\textbf{\textbar}\textbf{99.76}}          & \multicolumn{1}{c|}{16.89\textbf{\textbar}34.72\textbf{\textbar}67.35\textbf{\textbar}\textbf{78.04}}       & \multicolumn{1}{c|}{24.77\textbf{\textbar}74.84\textbf{\textbar}82.58\textbf{\textbar}\textbf{88.74}}        & \multicolumn{1}{c|}{31.10\textbf{\textbar}53.35\textbf{\textbar}74.77\textbf{\textbar}\textbf{80.42}}   & 99.10\textbf{\textbar}03.02\textbf{\textbar}98.70\textbf{\textbar}\textbf{99.21}          \\ \cline{2-7} 
%-----Drive Diagnosis---- 0.10 ----------------------------------
& \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{99.71\textbf{\textbar}93.90\textbf{\textbar} 99.76\textbf{\textbar}\textbf{99.79}}          & \multicolumn{1}{c|}{19.86\textbf{\textbar}35.27\textbf{\textbar} 58.79\textbf{\textbar}\textbf{66.13}}       & \multicolumn{1}{c|}{26.20\textbf{\textbar}70.99\textbf{\textbar} 78.07\textbf{\textbar}\textbf{83.59}}        & \multicolumn{1}{c|}{33.32\textbf{\textbar}52.29\textbf{\textbar} 69.50\textbf{\textbar}\textbf{75.30}}      & 98.58\textbf{\textbar}01.61\textbf{\textbar} 98.13\textbf{\textbar}\textbf{98.83}          \\ \hline
%--------------------  MNIST ------------------------------------                                                 
\multicolumn{1}{|c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}MNIST  \\ Dataset \\ ~\cite{data_gas} \\ \end{tabular}} }      & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{\textbf{97.81}\textbf{\textbar}96.41\textbf{\textbar} 97.13\textbf{\textbar}97.31 }          & \multicolumn{1}{c|}{82.79\textbf{\textbar}59.08\textbf{\textbar} 86.33\textbf{\textbar}\textbf{89.15} }       & \multicolumn{1}{c|}{80.14\textbf{\textbar}81.07\textbf{\textbar} 91.36\textbf{\textbar}\textbf{93.16} }        & \multicolumn{1}{c|}{79.55\textbf{\textbar}67.15\textbf{\textbar} 83.94\textbf{\textbar}\textbf{87.64} }         & 99.21\textbf{\textbar}80.72\textbf{\textbar} 99.64\textbf{\textbar}\textbf{99.72}         \\ \cline{2-7} 
%------------MNIST----- 0.30 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\textbf{97.69}\textbf{\textbar}96.07\textbf{\textbar} 97.19\textbf{\textbar}97.09}         & \multicolumn{1}{c|}{80.51\textbf{\textbar}54.99\textbf{\textbar} 87.35\textbf{\textbar}\textbf{89.46}}      & \multicolumn{1}{c|}{78.05\textbf{\textbar}78.16\textbf{\textbar}92.13\textbf{\textbar}\textbf{93.22}}        & \multicolumn{1}{c|}{79.39\textbf{\textbar}64.83\textbf{\textbar} 86.95\textbf{\textbar}\textbf{88.52}}        & 98.98\textbf{\textbar}58.04\textbf{\textbar}\textbf{99.10}\textbf{\textbar}98.94          \\ \cline{2-7} 
%----------MNIST---- 0.25 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{\textbf{97.68}\textbf{\textbar}99.63\textbf{\textbar} 97.16\textbf{\textbar}97.18}                & \multicolumn{1}{c|}{83.43\textbf{\textbar}46.49\textbf{\textbar} 82.16\textbf{\textbar}\textbf{89.12}}             & \multicolumn{1}{c|}{80.73\textbf{\textbar}75.07\textbf{\textbar}89.87\textbf{\textbar}\textbf{92.97}}              & \multicolumn{1}{c|}{80.98\textbf{\textbar}61.01\textbf{\textbar}83.63\textbf{\textbar}\textbf{88.08}   }           &\textbf{98.91}\textbf{\textbar}56.45\textbf{\textbar} 98.90\textbf{\textbar}98.81                       \\ \cline{2-7} 
%-----------MNIST--- 0.20 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{\textbf{97.74}\textbf{\textbar}95.99\textbf{\textbar} 97.28\textbf{\textbar}97.22}                & \multicolumn{1}{c|}{80.81\textbf{\textbar}54.23\textbf{\textbar} 87.46\textbf{\textbar}\textbf{89.93}}             & \multicolumn{1}{c|}{78.16\textbf{\textbar}77.48\textbf{\textbar} 86.48\textbf{\textbar}\textbf{93.49}}              & \multicolumn{1}{c|}{79.27\textbf{\textbar}65.65\textbf{\textbar}87.70\textbf{\textbar}\textbf{89.30}}              &98.10\textbf{\textbar}55.48\textbf{\textbar} 98.50\textbf{\textbar}  \textbf{98.56}            \\ \cline{2-7}
%----------MNIST----- 0.15 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{\textbf{97.73}\textbf{\textbar}96.01\textbf{\textbar} 97.05\textbf{\textbar}97.19}                & \multicolumn{1}{c|}{84.85\textbf{\textbar}55.02\textbf{\textbar} 82.50\textbf{\textbar}\textbf{87.72}}             & \multicolumn{1}{c|}{82.23\textbf{\textbar}78.15\textbf{\textbar} 89.41\textbf{\textbar}\textbf{92.52}}              & \multicolumn{1}{c|}{82.51\textbf{\textbar}66.59\textbf{\textbar} 83.80\textbf{\textbar}\textbf{88.41}}              & 98.06\textbf{\textbar}53.82\textbf{\textbar} 98.15\textbf{\textbar}\textbf{98.19}               \\ \cline{2-7}
%---------MNIST------ 0.10 ----------------------------------
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{\textbf{97.63}\textbf{\textbar}95.92\textbf{\textbar} 97.20\textbf{\textbar}97.16 }                & \multicolumn{1}{c|}{86.53\textbf{\textbar}51.44\textbf{\textbar} 86.25\textbf{\textbar}\textbf{88.77}}             & \multicolumn{1}{c|}{84.12\textbf{\textbar}76.54\textbf{\textbar} 91.56\textbf{\textbar}\textbf{92.81}}              & \multicolumn{1}{c|}{83.16\textbf{\textbar}63.44\textbf{\textbar} 86.47\textbf{\textbar}\textbf{88.58}}   &\textbf{97.33}\textbf{\textbar}41.66\textbf{\textbar} 97.05\textbf{\textbar}  96.81             \\ \hline
\end{tabular}
}
\end{table*}
% \end{table}




% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \begin{table}[]
% \begin{table*}%[hbt!]
% \resizebox{17.85cm}{!}
% {
% \begin{tabular}{|c|ccccccc|}
% \hline
% \multirow{3}{*}{Dataset}                          & \multicolumn{1}{c|}{MDR}  & \multicolumn{1}{c|}{\textbf{ID class}}       & \multicolumn{4}{c|}{\textbf{OOD class}}                                                                                                                                         &\textbf{Minority class} \\ \cline{2-8} 
% & \multicolumn{7}{c|}{Softmax ~\cite{softmax}\textbf{\textbar}Lee et. al. ~\cite{lee2018simple}\textbf{\textbar}Deep-MCDD ~\cite{deep_mcdd}\textbf{\textbar}DNN-GDID (ours)}                                                                                                                                                                                                            \\ \cline{2-8} 
% & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{Classification accuracy} & \multicolumn{1}{c|}{TNR at 85\% TPR}      & \multicolumn{1}{c|}{AUROC}                 & \multicolumn{1}{c|}{AUPR}                 & \multicolumn{1}{c|}{Detection accuracy}   & AUPR                    \\ \hline\hline
% % #-------------SYN FINANCIAL ------------------
% \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Synthetic \\ financial\\ Dataset\end{tabular}}               & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{\textbf{99.45}\textbf{\textbar}\textbf{\textbar} 99.31\textbf{\textbar}99.34}    & \multicolumn{1}{c|}{43.93\textbf{\textbar}\textbf{\textbar} 83.90\textbf{\textbar}\textbf{86.01}} & \multicolumn{1}{c|}{48.43\textbf{\textbar}\textbf{\textbar} 90.65\textbf{\textbar}\textbf{91.45}}  & \multicolumn{1}{c|}{86.12\textbf{\textbar}\textbf{\textbar}97.39\textbf{\textbar}\textbf{97.53}}   & \multicolumn{1}{c|}{66.26\textbf{\textbar}\textbf{\textbar}84.67\textbf{\textbar}\textbf{85.69}} & 98.59\textbf{\textbar}\textbf{\textbar} 99.31\textbf{\textbar}\textbf{99.33}    \\ \cline{2-8} 
% %-------SYN FINANCIAL---- 0.30 ----------------------------------
% & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\textbf{99.41}\textbf{\textbar}\textbf{\textbar} 99.21\textbf{\textbar}99.34}                & \multicolumn{1}{c|}{47.20\textbf{\textbar}\textbf{\textbar}84.36\textbf{\textbar}\textbf{89.09}}              & \multicolumn{1}{c|}{45.47\textbf{\textbar}\textbf{\textbar}  90.73\textbf{\textbar}93.22}             & \multicolumn{1}{c|}{86.97\textbf{\textbar}\textbf{\textbar}  97.69\textbf{\textbar}\textbf{98.34}}            & \multicolumn{1}{c|}{67.98\textbf{\textbar}\textbf{\textbar}84.99\textbf{\textbar}\textbf{87.69}}            & 95.87\textbf{\textbar}\textbf{\textbar}96.33\textbf{\textbar}\textbf{96.56}               \\ \cline{2-8}
% %---------SYN FINANCIAL--- 0.25 ----------------------------------
% & \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{\textbf{99.43}\textbf{\textbar}\textbf{\textbar}99.22\textbf{\textbar}99.34}           & \multicolumn{1}{c|}{44.99\textbf{\textbar}84.79\textbf{\textbar}\textbf{\textbar}\textbf{87.16}}       & \multicolumn{1}{c|}{45.40\textbf{\textbar}\textbf{\textbar} 90.29\textbf{\textbar}\textbf{92.13}}              & \multicolumn{1}{c|}{86.83\textbf{\textbar}\textbf{\textbar} 97.70\textbf{\textbar}\textbf{98.00}}              & \multicolumn{1}{c|}{66.89\textbf{\textbar}\textbf{\textbar}85.32\textbf{\textbar}\textbf{86.46}}             & 94.47\textbf{\textbar}\textbf{\textbar} 94.97\textbf{\textbar}\textbf{95.66}              \\ \cline{2-8} 
% %-------SYN FINANCIAL--- 0.20 ----------------------------------
% & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{99.44\textbf{\textbar}\textbf{\textbar} 99.28\textbf{\textbar}99.34}                & \multicolumn{1}{c|}{48.04\textbf{\textbar}\textbf{\textbar} 88.16\textbf{\textbar}84.58}             & \multicolumn{1}{c|}{47.55\textbf{\textbar}\textbf{\textbar} 92.66\textbf{\textbar}89.90}              & \multicolumn{1}{c|}{87.84\textbf{\textbar}\textbf{\textbar} 98.17\textbf{\textbar}97.58}              & \multicolumn{1}{c|}{69.12\textbf{\textbar}\textbf{\textbar}87.12\textbf{\textbar}85.19}             &94.70\textbf{\textbar}\textbf{\textbar} 93.85\textbf{\textbar}93.49               \\ \cline{2-8}
% %--------SYN FINANCIAL--- 0.15 ----------------------------------
% & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{99.52\textbf{\textbar}\textbf{\textbar} 99.37\textbf{\textbar}99.44}                & \multicolumn{1}{c|}{47.02\textbf{\textbar}\textbf{\textbar}86.38 \textbf{\textbar}84.71}             & \multicolumn{1}{c|}{45.94\textbf{\textbar}\textbf{\textbar} 91.36\textbf{\textbar}90.58}              & \multicolumn{1}{c|}{87.52\textbf{\textbar}\textbf{\textbar} 98.05\textbf{\textbar}97.73}              & \multicolumn{1}{c|}{69.33\textbf{\textbar}\textbf{\textbar} 86.20\textbf{\textbar}85.08}             &92.14\textbf{\textbar}\textbf{\textbar} 92.11\textbf{\textbar}90.86               \\ \cline{2-8} 
% %-------SYN FINANCIAL-- 0.10 ----------------------------------
% & \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{99.58\textbf{\textbar}\textbf{\textbar} 99.46\textbf{\textbar}99.49 }                & \multicolumn{1}{c|}{49.76\textbf{\textbar}\textbf{\textbar} 87.74\textbf{\textbar}85.10}             & \multicolumn{1}{c|}{48.67\textbf{\textbar}\textbf{\textbar} 92.67\textbf{\textbar}91.44}              & \multicolumn{1}{c|}{88.43\textbf{\textbar}\textbf{\textbar} 98.31\textbf{\textbar}97.89}              & \multicolumn{1}{c|}{70.11\textbf{\textbar}\textbf{\textbar}87.14 \textbf{\textbar}85.41}             & 90.10\textbf{\textbar}\textbf{\textbar}89.37\textbf{\textbar} 87.59              \\ \hline
% % #------------ GAS SENSOR --------------------
% \multicolumn{1}{|c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Gas \\ Sensor \\ Dataset \\ ~\cite{data_gas}\end{tabular}} } & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{\textbf{99.67}\textbf{\textbar}\textbf{\textbar} 99.61\textbf{\textbar} 99.66}     & \multicolumn{1}{c|}{45.59\textbf{\textbar}\textbf{\textbar} 93.13\textbf{\textbar}\textbf{97.62}} & \multicolumn{1}{c|}{60.24\textbf{\textbar}\textbf{\textbar} 95.88\textbf{\textbar}\textbf{97.59}}  & \multicolumn{1}{c|}{72.44\textbf{\textbar}\textbf{\textbar}  95.43\textbf{\textbar}\textbf{97.19}} & \multicolumn{1}{c|}{65.76\textbf{\textbar}\textbf{\textbar} 90.27\textbf{\textbar}\textbf{93.27}} & 99.61\textbf{\textbar}\textbf{\textbar}\textbf{99.63}\textbf{\textbar}99.60   \\ \cline{2-8} 
% %----------------------- GAS SENSOR-- 0.30 ------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\textbf{99.70}\textbf{\textbar}\textbf{\textbar} 99.69\textbf{\textbar}99.68}    & \multicolumn{1}{c|}{40.34\textbf{\textbar}\textbf{\textbar} 93.51\textbf{\textbar}\textbf{93.64}} & \multicolumn{1}{c|}{57.16\textbf{\textbar}\textbf{\textbar}  95.98\textbf{\textbar}\textbf{96.04}} & \multicolumn{1}{c|}{71.78\textbf{\textbar}\textbf{\textbar}\textbf{96.29}\textbf{\textbar}95.98}  & \multicolumn{1}{c|}{63.90\textbf{\textbar}\textbf{\textbar}\textbf{90.25}\textbf{\textbar}90.20} &\textbf{98.05}\textbf{\textbar}\textbf{\textbar} 97.69\textbf{\textbar}\textbf{98.05 }   \\ \cline{2-8} 
% %--------------- GAS SENSOR-- 0.25 -------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{99.68\textbf{\textbar}\textbf{\textbar}\textbf{99.70}\textbf{\textbar}99.68}    & \multicolumn{1}{c|}{40.02\textbf{\textbar}\textbf{\textbar} 93.69\textbf{\textbar}\textbf{94.15}} & \multicolumn{1}{c|}{56.13\textbf{\textbar}\textbf{\textbar} 95.88\textbf{\textbar}\textbf{96.07}}  & \multicolumn{1}{c|}{70.86\textbf{\textbar}\textbf{\textbar} 95.85\textbf{\textbar}\textbf{96.21}}  & \multicolumn{1}{c|}{63.28\textbf{\textbar}\textbf{\textbar} 90.46\textbf{\textbar}\textbf{91.00}} & 97.08\textbf{\textbar}\textbf{\textbar}\textbf{98.05}\textbf{\textbar}97.95    \\ \cline{2-8}
% %------------ GAS SENSOR--- 0.20 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{\textbf{99.68}\textbf{\textbar}\textbf{\textbar} 99.67\textbf{\textbar}99.64}    & \multicolumn{1}{c|}{45.16\textbf{\textbar}\textbf{\textbar}93.94\textbf{\textbar}\textbf{94.70}}  & \multicolumn{1}{c|}{60.36\textbf{\textbar}\textbf{\textbar} 96.00\textbf{\textbar}\textbf{96.62}}  & \multicolumn{1}{c|}{74.61\textbf{\textbar}\textbf{\textbar}96.09\textbf{\textbar}\textbf{96.51}}   & \multicolumn{1}{c|}{ 65.80\textbf{\textbar}\textbf{\textbar} 90.67\textbf{\textbar}\textbf{91.89}} & 97.44\textbf{\textbar}\textbf{\textbar}\textbf{97.59}\textbf{\textbar}97.35    \\ \cline{2-8} 
% %---------- GAS SENSOR--- 0.15 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{99.67\textbf{\textbar}\textbf{\textbar}\textbf{99.71}\textbf{\textbar}99.70}    & \multicolumn{1}{c|}{36.44\textbf{\textbar}\textbf{\textbar}84.34\textbf{\textbar}\textbf{96.61}} & \multicolumn{1}{c|}{57.20\textbf{\textbar}\textbf{\textbar} 92.35\textbf{\textbar}\textbf{97.11}}  & \multicolumn{1}{c|}{70.18\textbf{\textbar}\textbf{\textbar} 92.64\textbf{\textbar}\textbf{97.04}}  & \multicolumn{1}{c|}{61.59\textbf{\textbar}\textbf{\textbar}85.97\textbf{\textbar}\textbf{92.36}} &96.71\textbf{\textbar}\textbf{\textbar} 96.23\textbf{\textbar}\textbf{96.76}    \\ \cline{2-8} 
% %---------- GAS SENSOR--- 0.10 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{99.68\textbf{\textbar}\textbf{\textbar} 99.71\textbf{\textbar}\textbf{99.72}}          & \multicolumn{1}{c|}{41.76\textbf{\textbar}\textbf{\textbar} 84.34\textbf{\textbar}\textbf{93.99}}       & \multicolumn{1}{c|}{58.60\textbf{\textbar}\textbf{\textbar} 92.35\textbf{\textbar}\textbf{96.12}}        & \multicolumn{1}{c|}{72.06\textbf{\textbar}\textbf{\textbar} 92.64\textbf{\textbar}\textbf{96.28}}        & \multicolumn{1}{c|}{64.53\textbf{\textbar}\textbf{\textbar} 85.97\textbf{\textbar}\textbf{90.45}}       & 96.00\textbf{\textbar}\textbf{\textbar}\textbf{96.23}\textbf{\textbar}\textbf{96.23}          \\ \hline

% %--------------------  Drive Diagnosis ------------------------------------
% \multirow{6}{*}{{\begin{tabular}[c]{@{}c@{}} Drive \\ Diagnosis \\ Dataset \\ ~\cite{data_drive}\end{tabular}}}                  & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{99.70\textbf{\textbar}\textbf{\textbar} 99.76\textbf{\textbar}\textbf{99.81}}   & \multicolumn{1}{c|}{15.45\textbf{\textbar}\textbf{\textbar} 63.56\textbf{\textbar}\textbf{66.54}}       & \multicolumn{1}{c|}{23.52\textbf{\textbar}\textbf{\textbar}80.29\textbf{\textbar}\textbf{83.43}}        & \multicolumn{1}{c|}{28.82\textbf{\textbar}\textbf{\textbar} 70.31\textbf{\textbar}\textbf{71.44}}        & \multicolumn{1}{c|}{52.15\textbf{\textbar}\textbf{\textbar} 74.64\textbf{\textbar}\textbf{76.53}}       & 99.71\textbf{\textbar}\textbf{\textbar}99.83\textbf{\textbar}\textbf{ 99.85}        \\ \cline{2-8}
% %------Drive Diagnosis--- 0.30 ----------------------------------
% & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{99.73\textbf{\textbar}\textbf{\textbar} 99.79\textbf{\textbar}\textbf{99.82}}    & \multicolumn{1}{c|}{15.68\textbf{\textbar}\textbf{\textbar}60.33\textbf{\textbar}\textbf{70.08}}  & \multicolumn{1}{c|}{22.50\textbf{\textbar}\textbf{\textbar}  79.37\textbf{\textbar}\textbf{84.94}} & \multicolumn{1}{c|}{29.71\textbf{\textbar}\textbf{\textbar}  69.98\textbf{\textbar}\textbf{74.47}} & \multicolumn{1}{c|}{52.03\textbf{\textbar}\textbf{\textbar} 73.65\textbf{\textbar}\textbf{78.27}} & 99.48\textbf{\textbar}\textbf{\textbar} 99.43\textbf{\textbar}\textbf{99.53}     \\ \cline{2-8} 
% %---Drive Diagnosis---- 0.25 ----------------------------------
% & \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{99.70\textbf{\textbar}\textbf{\textbar} 99.78\textbf{\textbar}\textbf{99.79}}          & \multicolumn{1}{c|}{16.19\textbf{\textbar}\textbf{\textbar} 53.79\textbf{\textbar}\textbf{64.90}}       & \multicolumn{1}{c|}{22.39\textbf{\textbar}\textbf{\textbar} 75.31\textbf{\textbar}\textbf{82.85}}        & \multicolumn{1}{c|}{30.02\textbf{\textbar}\textbf{\textbar} 66.13\textbf{\textbar}\textbf{71.94}}        & \multicolumn{1}{c|}{22.39\textbf{\textbar}\textbf{\textbar} 70.22\textbf{\textbar}\textbf{75.82}}       & 98.96\textbf{\textbar}\textbf{\textbar} 99.47\textbf{\textbar}\textbf{99.48 }        \\ \cline{2-8} 
% %-------Drive Diagnosis---- 0.20 ----------------------------------
% & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{99.73\textbf{\textbar}\textbf{\textbar} 99.79\textbf{\textbar}\textbf{99.81}}          & \multicolumn{1}{c|}{17.79\textbf{\textbar}\textbf{\textbar} 66.61\textbf{\textbar}\textbf{70.20}}       & \multicolumn{1}{c|}{26.48\textbf{\textbar}\textbf{\textbar}82.97\textbf{\textbar}\textbf{85.44}}        & \multicolumn{1}{c|}{32.51\textbf{\textbar}\textbf{\textbar} 74.30\textbf{\textbar}\textbf{75.76}}        & \multicolumn{1}{c|}{52.91\textbf{\textbar}\textbf{\textbar} 76.43\textbf{\textbar}\textbf{78.20}}       & 98.75\textbf{\textbar}\textbf{\textbar}\textbf{99.33}\textbf{\textbar}99.32          \\ \cline{2-8} 
% %------Drive Diagnosis----- 0.15 ----------------------------------
% & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{99.70\textbf{\textbar}\textbf{\textbar} 99.74\textbf{\textbar}\textbf{99.80}}          & \multicolumn{1}{c|}{16.89\textbf{\textbar}\textbf{\textbar}\textbf{67.35}\textbf{\textbar}59.88}       & \multicolumn{1}{c|}{24.77\textbf{\textbar}\textbf{\textbar}\textbf{82.58}\textbf{\textbar}80.91}        & \multicolumn{1}{c|}{31.10\textbf{\textbar}\textbf{\textbar}\textbf{74.77}\textbf{\textbar}70.08}        & \multicolumn{1}{c|}{52.12\textbf{\textbar}\textbf{\textbar}\textbf{76.75}\textbf{\textbar} 73.66}       & 99.10\textbf{\textbar}\textbf{\textbar}98.70\textbf{\textbar}\textbf{99.21}          \\ \cline{2-8} 
% %-----Drive Diagnosis---- 0.10 ----------------------------------
% & \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{99.71\textbf{\textbar}\textbf{\textbar} 99.76\textbf{\textbar}\textbf{99.79}}          & \multicolumn{1}{c|}{19.86\textbf{\textbar}\textbf{\textbar} 58.79\textbf{\textbar}\textbf{66.13}}       & \multicolumn{1}{c|}{26.20\textbf{\textbar}\textbf{\textbar} 78.07\textbf{\textbar}\textbf{83.59}}        & \multicolumn{1}{c|}{33.32\textbf{\textbar}\textbf{\textbar} 69.50\textbf{\textbar}\textbf{75.30}}        & \multicolumn{1}{c|}{53.37\textbf{\textbar}\textbf{\textbar} 72.81\textbf{\textbar}\textbf{76.55}}       & 98.58\textbf{\textbar}\textbf{\textbar} 98.13\textbf{\textbar}\textbf{98.83}          \\ \hline
% %--------------------  MNIST ------------------------------------                                                 
% \multicolumn{1}{|c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}MNIST  \\ Dataset \\ ~\cite{data_gas} \\ \end{tabular}} }      & \multicolumn{1}{c|}{1.00} & \multicolumn{1}{c|}{\textbf{97.81}\textbf{\textbar}\textbf{\textbar} 97.13\textbf{\textbar}97.31 }          & \multicolumn{1}{c|}{82.79\textbf{\textbar}\textbf{\textbar} 86.33\textbf{\textbar}\textbf{89.15} }       & \multicolumn{1}{c|}{80.14\textbf{\textbar}\textbf{\textbar} 91.36\textbf{\textbar}\textbf{93.16} }        & \multicolumn{1}{c|}{79.55\textbf{\textbar}\textbf{\textbar} 83.94\textbf{\textbar}\textbf{87.64} }        & \multicolumn{1}{c|}{86.47\textbf{\textbar}\textbf{\textbar} 85.81\textbf{\textbar}\textbf{87.32} }       & 99.21\textbf{\textbar}\textbf{\textbar} 99.64\textbf{\textbar}\textbf{99.72}         \\ \cline{2-8} 
% %------------MNIST----- 0.30 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\textbf{97.69}\textbf{\textbar}\textbf{\textbar} 97.19\textbf{\textbar}97.09}         & \multicolumn{1}{c|}{80.51\textbf{\textbar}\textbf{\textbar} 87.35\textbf{\textbar}\textbf{89.46}}      & \multicolumn{1}{c|}{78.05\textbf{\textbar}92.13\textbf{\textbar}\textbf{\textbar}\textbf{93.22}}        & \multicolumn{1}{c|}{79.39\textbf{\textbar}\textbf{\textbar} 86.95\textbf{\textbar}\textbf{88.52}}       & \multicolumn{1}{c|}{85.79\textbf{\textbar}\textbf{\textbar} 86.35\textbf{\textbar}\textbf{87.46}}      & 98.98\textbf{\textbar}\textbf{\textbar}\textbf{99.10}\textbf{\textbar}98.94          \\ \cline{2-8} 
% %----------MNIST---- 0.25 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.25} & \multicolumn{1}{c|}{97.68\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}97.18}                & \multicolumn{1}{c|}{83.43\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}89.12}             & \multicolumn{1}{c|}{80.73\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}92.97}              & \multicolumn{1}{c|}{80.98\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}88.08}              & \multicolumn{1}{c|}{86.74\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}87.27}             &  98.91\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}98.81                       \\ \cline{2-8} 
% %-----------MNIST--- 0.20 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{97.74\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}97.22}                & \multicolumn{1}{c|}{80.81\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}89.93}             & \multicolumn{1}{c|}{78.16\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}93.49}              & \multicolumn{1}{c|}{79.27\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}89.30}              & \multicolumn{1}{c|}{85.36\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}87.81}             & 98.10\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}   98.56            \\ \cline{2-8}
% %----------MNIST----- 0.15 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{97.73\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}97.19}                & \multicolumn{1}{c|}{84.85\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}87.72}             & \multicolumn{1}{c|}{82.23\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}92.52}              & \multicolumn{1}{c|}{82.51\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}88.41}              & \multicolumn{1}{c|}{87.55\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}86.61 }             &98.06\textbf{\textbar}\textbf{\textbar}\textbf{\textbar}98.19               \\ \cline{2-8}
% %---------MNIST------ 0.10 ----------------------------------
% \multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{0.10} & \multicolumn{1}{c|}{\textbf{97.63}\textbf{\textbar}\textbf{\textbar} 97.20\textbf{\textbar}97.16 }                & \multicolumn{1}{c|}{86.53\textbf{\textbar}\textbf{\textbar} 86.25\textbf{\textbar}\textbf{88.77}}             & \multicolumn{1}{c|}{84.12\textbf{\textbar}\textbf{\textbar} 91.56\textbf{\textbar}\textbf{92.81}}              & \multicolumn{1}{c|}{83.16\textbf{\textbar}\textbf{\textbar} 86.47\textbf{\textbar}\textbf{88.58}}              & \multicolumn{1}{c|}{\textbf{87.63}\textbf{\textbar}\textbf{\textbar} 85.74\textbf{\textbar}87.09}             &\textbf{97.33}\textbf{\textbar}\textbf{\textbar} 97.05\textbf{\textbar}  96.81             \\ \hline
% \end{tabular}
% }
% \vspace{0.2cm}
% \caption{Comparison of our proposed algorithm (DNN-GDID) with Softmax ~\cite{softmax},K Lee et al. ~\cite{lee2018simple} and Deep-MCDD ~\cite{deep_mcdd}. Best performance is highlighted in bold.}
% \label{table_class}
% \end{table*}
% % \end{table}
